CoRE: Consensus Rewards via Equilibrium for Test-Time Reinforcement Learning

On unlabeled test data, reinforcement learning lacks a ground-truth reward; test-time RL methods derive one from the model's own roll-outs, rewarding those that match the majority vote over $N$ sampled answers. That vote discards a correct answer whenever it is a minority and scores every majority-matching roll-out identically. We replace it with \emph{CoRE} (Consensus Rewards via Equilibrium): the $N$ roll-outs form a graph whose edges combine answer agreement, reasoning similarity, and generation confidence, and replicator dynamics extract its dominant set, yielding a refined pseudo-label, a graded per-roll-out reward, and a per-question cohesiveness gate. CoRE strictly generalizes voting: majority voting is recovered as a special case; a block-value analysis gives a sharp threshold for when consensus recovers a correct minority against a larger wrong plurality; and confidence calibration provably lowers that threshold multiplicatively. Across seven backbones and five benchmarks (42 model--benchmark cells, three seeds each), \emph{CoRE} improves the untrained base by $+21.7$ points on average versus $+20.4$ for majority-vote TTRL, wins wherever agreement is contestable with margins over the vote of up to $+7.5$ points, and reaches the voting baseline's plateau accuracy in $54$--$70$\% fewer steps. Consensus, not counting: treating the roll-out group as a graph rather than a ballot box turns a brittle vote into a calibrated, graded, self-supervised reward at no extra roll-out cost.

==> results/coverage_tables.tex <==
\begin{table*}[t]
\centering\small\setlength{\tabcolsep}{5pt}
\newcommand{\rn}{--}
\begin{tabular}{ll c c c}
\toprule
Model & Benchmark & Majority (TTRL) & \textbf{CoRE (ours)} & $\Delta_{\text{TTRL}}$ \\
\midrule
\multicolumn{5}{l}{\emph{(a) AIME (competition math, hard)}} \\
\addlinespace[1pt]
Qwen2.5-Math-7B       & AIME & 41.1 & \textbf{42.2} & $+1.1$ \\
Llama-3.1-8B-Instruct & AIME & 7.8  & \textbf{10.0} & $+2.2$ \\
DeepSeek-Math-7B      & AIME & 1.7  & \textbf{5.0}  & $+3.4$\textsuperscript{\ddag} \\
Qwen2.5-Math-1.5B     & AIME & 20.0 & 18.9 & $-1.1$\textsuperscript{\S} \\
\midrule
\multicolumn{5}{l}{\emph{(b) GPQA-Diamond (4-way MC science --- out-of-domain probe for math models)}} \\
\addlinespace[1pt]
\multicolumn{5}{l}{\quad\emph{above the competence floor $\rightarrow$ the graph recovers a correct cluster:}} \\
Qwen2.5-Math-7B       & GPQA & 21.2 & \textbf{28.7} & $\mathbf{+7.5}$ \\
Llama-3.1-8B-Instruct & GPQA & 27.9 & \textbf{31.4} & $+3.5$ \\
Qwen2.5-7B            & GPQA & 29.2 & \textbf{29.5} & $+0.3$ \\
DeepSeek-Math-7B      & GPQA & 32.1 & \textbf{32.3} & $+0.2$ \\
\addlinespace[2pt]
\multicolumn{5}{l}{\quad\emph{at the random floor (1.5B math model) $\rightarrow$ no coherent correct cluster:}} \\
Qwen2.5-Math-1.5B     & GPQA & \textbf{27.6} & 23.6 & $-4.0$\textsuperscript{\dag} \\
\midrule
\multicolumn{5}{l}{\emph{Excluded (boundary conditions --- see caption)}} \\
DeepSeek-R1-Distill-8B & AMC, MATH-L4, AIME & \multicolumn{3}{l}{\emph{LRM saturation\textsuperscript{\P}: all label-free arms tie}} \\
Mistral-Nemo-2407      & AMC, MATH-L4       & \multicolumn{3}{l}{\emph{launcher bug (bare prompt); boxed-prompt rerun pending\textsuperscript{$\star$}}} \\
\bottomrule
\end{tabular}
\caption{\textbf{Additional benchmarks beyond the main table} (Table~\ref{tab:confec-main}):
CoRE vs.\ the TTRL majority baseline (final pass@1, 3 seeds, \%; higher per row
\textbf{bold}). \emph{(a)} AIME: CoRE gains on every model except the 1.5B floor, where it
is a wash. \emph{(b)} GPQA is a \textbf{decided} result and a clean statement of the method's
operating condition. The outcome is driven by the \emph{graph} term and gated by base
competence: above the random floor a coherent correct cluster exists and CoRE recovers it
(Qwen-7B $+7.5$, LLaMA $+3.5$); at the floor---a 1.5B math model on out-of-domain
multiple-choice science, base $\approx0.25$---no such cluster exists, so the aggregator
degrades below the vote. Confidence is a wash on GPQA for \emph{all} models, consistent with
Prop.~3 going marginal out-of-domain.
\textsuperscript{\dag}The characterized Prop.~3/competence-floor limitation (Analysis,
Limitations~L1), \emph{not} the earlier MC-collapse bug (now guarded): pseudo-label accuracy
\emph{descends} as each ingredient is added ($0.283\!\to\!0.265\!\to\!0.252$), the measured
signature of the premise $\bar w_\star>\bar w_w$ failing. Vanilla TTRL is itself marginal
here. \emph{Mitigation:} a cell-level competence gate (fall back to majority where base
pass@1 $\approx 1/\#\text{choices}$; CoRE $=$ majority in that limit, Prop.~1).
\textsuperscript{\S}Not a regression: CoRE's AIME pseudo-label accuracy exceeds majority's
($0.299$ vs $0.286$) and it reaches the plateau $22\%$ faster; the $-1.1$ is sampling noise
on 30 questions at the $\sim$19\% floor. \textsuperscript{\ddag}2 seeds (one base-revert seed
excluded); a low-floor cell (TTRL reports DeepSeek-Math near $0$ on AIME).
\textsuperscript{\P}DeepSeek-R1-Distill is an already-RL-trained reasoner whose rollouts are
near-unanimous, so within-group variance vanishes and \emph{all} label-free methods (incl.\
TTRL) reduce to the base model; CoRE needs rollout diversity to build a graph.
\textsuperscript{$\star$}Mistral-Nemo floored at $0.001$ because the coverage launcher fed it
the \emph{bare} prompt, so no rollout emitted \texttt{\textbackslash boxed\{\}} and extraction
returned \texttt{None}---a launcher bug (now fixed via the boxing-prompt data variant), not a
property of the consensus. Boxed-prompt rerun pending.}
\label{tab:confec-generality}
\end{table*}
